Deposit of Red Blood Cells at low concentrations in evaporating droplets: central edge growth and potential applications

Evaporation of blood droplets and diluted blood samples is a topic of intensive research, as it is seen as a possible low-cost tool for diagnosis. So far, samples with volume fraction down to a few percents of Red Blood Cells (RBCs) have been studied, and those were reportedly dominated by a ``coffee-ring'' deposit. In this study, samples with lower volume fractions have been used in order to study the growth of the evaporative deposit from sessile droplets more in details. We observed that blood samples and salt solutions with less than 1\% volume fraction of RBCs are dominated by a central deposit. We characterized the growth process of this central deposit by evaporating elongated drops, and determined that it is consistent with the Kardar-Parisi-Zhang process in the presence of quenched disorder. Our results showed a sensitivity of this deposit size to the fibrinogen concentration and shape of the RBCs, meaning that this parameter could be used to develop a new and cost-effective clinical marker for inflammation and RBC deformation.

==> BiblioBloodDrop.tex <==
@article{sikarwar2016automatic,
  title={Automatic disease screening method using image processing for dried blood microfluidic drop stain pattern recognition},
  author={Sikarwar, Basant S and Roy, Mukesh and Ranjan, Priya and Goyal, Ayush},
  journal={Journal of medical engineering \& technology},
  volume={40},
  number={5},
  pages={245--254},
  year={2016},
  publisher={Taylor \& Francis}
}

@article{bahmani2017study,
  title={The study of drying and pattern formation of whole human blood drops and the effect of thalassaemia and neonatal jaundice on the patterns},
  author={Bahmani, Leila and Neysari, Mahdi and Maleki, Maniya},
  journal={Colloids and Surfaces A: Physicochemical and Engineering Aspects},
  volume={513},
  pages={66--75},
  year={2017},
  publisher={Elsevier}
}

@article{liu2020automatic,
  title={Automatic classification of bloodstain patterns caused by gunshot and blunt impact at various distances},
  author={Liu, Yu and Attinger, Daniel and De Brabanter, Kris},
  journal={Journal of forensic sciences},
  volume={65},
  number={3},
  pages={729--743},
  year={2020},
  publisher={Wiley Online Library}
}

@article{attinger2022using,
  title={Using the likelihood ratio in bloodstain pattern analysis},
  author={Attinger, Daniel and De Brabanter, Kris and Champod, Christophe},
  journal={Journal of Forensic Sciences},
  volume={67},
  number={1},
  pages={33--43},
  year={2022},
  publisher={Wiley Online Library}
}

@article{deegan1997capillary,
  title={Capillary flow as the cause of ring stains from dried liquid drops},
  author={Deegan, Robert D and Bakajin, Olgica and Dupont, Todd F and Huber, Greb and Nagel, Sidney R and Witten, Thomas A},
  journal={Nature},
  volume={389},
  number={6653},
  pages={827--829},
  year={1997},
  publisher={Nature Publishing Group UK London}
}

@article{rossi2019interfacial,
  title={Interfacial flows in sessile evaporating droplets of mineral water},
  author={Rossi, Massimiliano and Marin, Alvaro and K{\"a}hler, Christian J},
  journal={Physical Review E},
  volume={100},
  number={3},
  pages={033103},
  year={2019},
  publisher={APS}
}

@article{darras2019combined,
  title={Combined effects of Marangoni, sedimentation and coffee-ring flows on evaporative deposits of superparamagnetic colloids},
  author={Darras, Alexis and Vandewalle, Nicolas and Lumay, Geoffroy},
  journal={Colloid and Interface Science Communications},
  volume={32},
  pages={100198},
  year={2019},
  publisher={Elsevier}
}

@article{darras2018transitional,
  title={Transitional bulk-solutal Marangoni instability in sessile drops},
  author={Darras, Alexis and Vandewalle, Nicolas and Lumay, Geoffroy},
  journal={Physical Review E},
  volume={98},
  number={6},
  pages={062609},
  year={2018},
  publisher={APS}
}

@article{zeid2013influence,
  title={Influence of relative humidity on spreading, pattern formation and adhesion of a drying drop of whole blood},
  author={Zeid, W Bou and Brutin, David},
  journal={Colloids and Surfaces A: Physicochemical and Engineering Aspects},
  volume={430},
  pages={1--7},
  year={2013},
  publisher={Elsevier}
}

@article{chen2016blood,
  title={Blood drop patterns: Formation and applications},
  author={Chen, Ruoyang and Zhang, Liyuan and Zang, Duyang and Shen, Wei},
  journal={Advances in colloid and interface science},
  volume={231},
  pages={1--14},
  year={2016},
  publisher={Elsevier}
}

@article{lanotte2017role,
  title={Role of red cells and plasma composition on blood sessile droplet evaporation},
  author={Lanotte, Luca and Laux, Didier and Charlot, Beno{\^\i}t and Abkarian, Manouk},
  journal={Physical Review E},
  volume={96},
  number={5},
  pages={053114},
  year={2017},
  publisher={APS}
}

@article{yunker2011suppression,
  title={Suppression of the coffee-ring effect by shape-dependent capillary interactions},
  author={Yunker, Peter J and Still, Tim and Lohr, Matthew A and Yodh, AG},
  journal={nature},
  volume={476},
  number={7360},
  pages={308--311},
  year={2011},
  publisher={Nature Publishing Group UK London}
}

@article{liu2019segregation,
  title={Segregation in drying binary colloidal droplets},
  author={Liu, Wendong and Midya, Jiarul and Kappl, Michael and Butt, Hans-Jürgen and Nikoubashman, Arash},
  journal={ACS nano},
  volume={13},
  number={5},
  pages={4972--4979},
  year={2019},
  publisher={ACS Publications}
}

@article{yunker2013effects,
  title={Effects of particle shape on growth dynamics at edges of evaporating drops of colloidal suspensions},
  author={Yunker, Peter J and Lohr, Matthew A and Still, Tim and Borodin, Alexei and Durian, Douglas J and Yodh, Arjun G},
  journal={Physical review letters},
  volume={110},
  number={3},
  pages={035501},
  year={2013},
  publisher={APS}
}

@article{pal2020concentration,
  title={Concentration-driven phase transition and self-assembly in drying droplets of diluting whole blood},
  author={Pal, Anusuya and Gope, Amalesh and Obayemi, John D and Iannacchione, Germano S},
  journal={Scientific reports},
  volume={10},
  number={1},
  pages={18908},
  year={2020},
  publisher={Nature Publishing Group UK London}
}

@article{pal2021temperature,
  title={Temperature and concentration dependence of human whole blood and protein drying droplets},
  author={Pal, Anusuya and Gope, Amalesh and Iannacchione, Germano},
  journal={Biomolecules},
  volume={11},
  number={2},
  pages={231},
  year={2021},
  publisher={MDPI}
}

@book{barabasi_stanley_1995,
  title={Fractal concepts in surface growth},
  author={Barab{\'a}si, A-L and Stanley, Harry Eugene},
  year={1995},
  publisher={Cambridge university press}
}

@article{FAMILY1990561,
  title={Dynamic scaling and phase transitions in interface growth},
  author={Family, Fereydoon},
  journal={Physica A: Statistical Mechanics and its Applications},
  volume={168},
  number={1},
  pages={561--580},
  year={1990},
  publisher={Elsevier}
}

@article{family1985scaling,
  title={Scaling of the active zone in the Eden process on percolation networks and the ballistic deposition model},
  author={Family, Fereydoon and Vicsek, Tamas},
  journal={Journal of Physics A: Mathematical and General},
  volume={18},
  number={2},
  pages={L75},
  year={1985},
  publisher={IOP Publishing}
}

@article{marin2019solutal,
  title={Solutal Marangoni flow as the cause of ring stains from drying salty colloidal drops},
  author={Marin, Alvaro and Karpitschka, Stefan and Noguera-Mar{\'\i}n, Diego and Cabrerizo-V{\'\i}lchez, Miguel A and Rossi, Massimiliano and K{\"a}hler, Christian J and Valverde, Miguel A Rodr{\'\i}guez},
  journal={Physical review fluids},
  volume={4},
  number={4},
  pages={041601},
  year={2019},
  publisher={APS}
}

@article{darras2018remote,
  title={Remote-controlled deposit of superparamagnetic colloidal droplets},
  author={Darras, Alexis and Mignolet, Florence and Vandewalle, Nicolas and Lumay, Geoffroy},
  journal={Physical Review E},
  volume={98},
  number={6},
  pages={062608},
  year={2018},
  publisher={APS}
}

@article{dasanna2022erythrocyte,
  title={Erythrocyte sedimentation: Effect of aggregation energy on gel structure during collapse},
  author={Dasanna, Anil Kumar and Darras, Alexis and John, Thomas and Gompper, Gerhard and Kaestner, Lars and Wagner, Christian and Fedosov, Dmitry A},
  journal={Physical Review E},
  volume={105},
  number={2},
  pages={024610},
  year={2022},
  publisher={APS}
}

@article{darras2023erythrocyte,
  title={Erythrocyte Sedimentation Rate: A Physics-Driven Characterization in a Medical Context},
  author={Darras, Alexis and John, Thomas and Wagner, Christian and Kaestner, Lars},
  journal={JoVE (Journal of Visualized Experiments)},
  number={193},
  pages={e64502},
  year={2023}
}

@article{john2024early,
  title={Early stage of erythrocyte sedimentation rate test: Fracture of a high-volume-fraction gel},
  author={John, Thomas and Kaestner, Lars and Wagner, Christian and Darras, Alexis},
  journal={PNAS nexus},
  volume={3},
  number={1},
  pages={pgad416},
  year={2024},
  publisher={Oxford University Press US}
}

@article{family1985scaling,
  title={Scaling of the active zone in the Eden process on percolation networks and the ballistic deposition model},
  author={Family, Fereydoon and Vicsek, Tamas},
  journal={Journal of Physics A: Mathematical and General},
  volume={18},
  number={2},
  pages={L75},
  year={1985},
  publisher={IOP Publishing}
}
@article{sardari2024,
    author = {Sardari, Vahideh and Safari, Fatemeh and Maleki, Maniya},
    title = "{Dynamics of the surface growth resulted from sedimentation of spheres in a Heleâ€“Shaw cell containing a low-viscosity fluid}",
    journal = {Physics of Fluids},
    volume = {36},
    number = {5},
    pages = {053303},
    year = {2024},
    month = {05},
    issn = {1070-6631},
    doi = {10.1063/5.0200886},
     publisher={AIP Publishing},
}
